Texts or Images? A Fine-grained Analysis on the Effectiveness of Input Representations and Models for Table Question Answering

In table question answering (TQA), tables are encoded as either texts or images. Prior work suggests that passing images of tables to multi-modal large language models (MLLMs) performs comparably to or even better than using textual input with large language models (LLMs). However, the lack of controlled setups limits fine-grained distinctions between these approaches. In this paper, we conduct the first controlled study on the effectiveness of several combinations of table representations and models from two perspectives: question complexity and table size. We build a new benchmark based on existing TQA datasets. In a systematic analysis of seven pairs of MLLMs and LLMs, we find that the best combination of table representation and model varies across setups. We propose FRES, a method selecting table representations dynamically, and observe a 10% average performance improvement compared to using both representations indiscriminately.

==> latex/old_chapters.tex <==
%\section{Experiments}
%\label{sec:experiments}
%


% \section{Improving MLLM Performance on Large Tables}
% \label{relevant_table}
% Our analysis \red{in Sec. 3} revealed that MLLMs struggle with processing large table images, but also that they exhibit superior table reasoning capabilities.\annetodo{any idea why that is the case?}
% % explained from lin 290-293, maybe because of the continue training with multimodal data. 
% While providing table text to MLLMs can mitigate the difficulties associated with large table inputs, it is not an optimal solution, as usually not all table cells are relevant to the question being asked.
% Additionally, longer input lengths can lead to higher inference time.
% In this section, we address two key questions to improve MLLM efficiency and performance when processing large tables: 1) How can we extract relevant cells from the tables? 2) How can we reintegrate this relevant cell information back to the model?\annetodo{this reintegration question seems a bit trivial, is it just prompt engineering?}
% % yes :) 

% \subsection{Sub-table Retrieval}
% We define a table $T$ as comprising a set of headers $H$, values $V$, and a schema function $S$ that maps values to their corresponding headers. Since a table can feature both top headers $ht$ and left headers $hl$, we represent the header set $H$ as $\{\emptyset, \{ht_1, \dots, ht_m\}\} \cup \{\emptyset, \{hl_1, \dots, hl_n\}\}$, where $m$ and $n$ represent the number of columns and rows, respectively. We use $ \emptyset$  to denote the absence of a header. For instance, the header representation for a flat table without left headers (we do not consider numerical indices as meaningful headers) is $\{ht_1, \dots, ht_m\}$. 
% The task of sub-table retrieval involves locating \textcolor{red}{relevant top headers, $th_{rel}$, relevant left headers $lh_{rel}$, and a set of cell values $V_{rel}$ indexed by those headers}\annetodo{a bit unclear: you locate the cells or the headers? is returning the headers mainly a by-product of identifying the cells, or is it a difficult task? introducing + explaining may make sense here} based on a question $ Q$ and a table $T$. 
% This can be mathematically represented as:
% $T' = \{V_{rel}, th_{rel}, lh_{rel} \mid Q, T \}$, where $V_{rel} = [\{v\}, v \in V, S(v) \in \{th_{rel}, lf_{rel}\}]$.


% \paragraph{System.} For a table that contains both top and left headers,  we leverage an LLM to select relevant headers: $hl_{rel} = LLM(Q, hl)$ and $ht_{rel} = LLM(Q, ht)$. Relevant cells are indexed by relevant headers. 
% In cases of flat tables where left headers are absent, the sub-table generated by only filtering columns can still be extensive if many rows are involved. To address this, \textcolor{red}{we select relevant rows based on filtering conditions generated by an LLM.: the LLM takes in a question and returns filtering conditions. Based on the conditions, it generates corresponding Python pandas code that is executed on the table. Header semantics matching is then conducted and operated on those filtered rows to obtain a sub-table. We also add back rows and columns where question tokens appear (henceforth, heuristic rows/cols) to make sure relevant information is contained in a sub-table. An example is shown in Figure \ref{fig:system}.} \annetodo{say what the input is + that the MLLM does that} %

% %\annetodo{pandas?} 
% % In our initial experiments, we find sometimes the generated sub-tables still lack relevant information. Consider the question \enquote{Which country won after France?} The filtered table does not contain the row featuring the performance of France anymore. Passing the filtered table can result in question being unanswerable. To solve this, we heuristically add back row and columns in which a question token appears. In this case, 
% %\annetodo{I do not quite understand this step: does it mean the filtering based on the MLLM-generated filters is too aggressive? how would this heuristic help to get the country that won after France?}.
% \annetodo{the example in Fig. 3 is not extremely well-chosen as the first step selects all the columns. I am somewhat unsure about the heuristic column selection step, can we discuss this? wouldn't it make sense to at least include the rows +/- 2 or something?}
% %will change the example and figure in the end. 

% Our approach, compared to methods that rely solely on header semantic matching, further reduces the number of relevant cells by generating and executing the filtering conditions. In contrast to approaches that use LLMs to directly return relevant row indices, our method provides more accurate matching as executing code through a program interpreter yields more reliable results than directly using an LLM, which is prone to generating incorrect or fabricated outputs. In cases where code execution results in errors, we revert to using results from header semantics matching, which also already outputs sub-tables.
% Prompts for parsing questions into filtering conditions and code generation can be found in \ref{prompts}.
% \paragraph{Ground truth Relevant Cells}
% For HiTab, the gold relevant cells are determined from the annotations provided in the dataset. Specifically, the annotated \textit{linked cells} are considered relevant. The gold top headers are identified as the first row. Since not all gold sub-tables have left headers, we treat them as flat tables. For other datasets where no annotations for relevant cells are available, we employ GPT-4 to identify the target columns and then progressively reason to pinpoint target rows before returning the answer. Prompts can be found in \ref{prompts}.
% Subsequently, we focus on instances where the prediction is accurate and use the predicted target columns and rows to construct sub-tables. For cases where the predicted answer is incorrect, or the resultant target table is excessively large (i.e., more than 10 rows), we manually review and refine them to create sub-tables. On average, approximately 82\% of cells are filtered out during this process.\annetodo{what is the accuracy of annotating the relevant cells using GPT4?}
% % there is no gold relevant cells to calculate this... (maybe do it on hitab?)

% \paragraph{Comparing baselines.}
% We compare our approach to two state-of-the-art (SoTA) systems that generate sub-tables: TableRAG \citep{Chen2024TableRAGMT} and GraphOTTER \cite{Li2024GraphOTTEREL}. TableRAG selects relevant table headers and values by prompting LLMs to generate natural language queries. These queries are then used to identify relevant headers and values. GraphOTTER, on the other hand, is tailored for hierarchical tables and utilizes LLMs to directly generate relevant cells and their indices.
% To estimate the upper and lower bounds of these systems, we use the overlapping set of all predicted columns and cells for the upper bound and consider only the predicted cells for the lower bound. For instance, if a system predicts a cell with an index (4,2), we include all cells in row 4 and column 2 for the upper bound and only the single predicted cell for the lower bound. These two methods are referred to as \textit{all} selection  and \textit{cell} selection, respectively.
% Additionally, we use the original, full table, which has a high recall rate, as another baseline for comparison.

% \paragraph{Results}
% We present the results for cell matching and top header matching in Table \ref{tab:sub_table_results}. All systems involving LLMs are powered by Qwen2 72b \cite{Yang2024Qwen2TR}. Our proposed method achieves the highest $F_1$ scores for both cell and top header matching. We observe that GraphOTTER tends to generate too few relevant cells, resulting in high precision but low recall. In contrast, TableRAG often generates an excessive number of headers, which explains why the system demonstrates high recall when adding predicted column values to the predicted cells (\textit{all} selection).
% Unlike these systems, our proposed method achieves high recall while maintaining good precision. It is noteworthy that the header recall of the ORI system is not 100\%; this is due to the gold target header from the HiTab dataset, where no cells are selected from the top headers in some instances.
% Analysis of our sub-table retriever can be found in the Appendix (ablation study? ablate parse q, ablate coder, ablate row indexing fully, ablate heuristic?)
% % TODO: add additional baseline for tabsqaulify (since it also generates code, SQL if have time)
% % difference to Tabsqualify: parsing can help generates more flexible and correct filtering condition for multi-step reasoning question: how many times did spain win after France? needs to first find out when France win and filter for spain win after that year, hard for SQL to generate, however, our parser can specify the complex step for the code generator and generate step by step.

% \begin{table}[htb]
%     \footnotesize
%     \centering    
%     \begin{tabular}{*{8}{c}}
%     \toprule
%     Model &  \multicolumn{3}{c}{Cell} &  \multicolumn{3}{c}{Top Header} &\# Extr. \\
%     & $p$& $r$& $F_1$ & $p$ & $r$ & $F_1$& Cells\\
%     \midrule
%     GO-all& 52& 53& 46 & 57 & 63 & 58&2.7 \\
%      GO-cell&\textbf{57} & 41 &43 & 57 & 63 &58&4.1\\
%     TRAG-all & 19 & 92 & 27& 39 & 74&48&9.3 \\
%     TRAG-cell &29 & 35 &26 & 39 & 74& 48&11 \\
%     ORI &21 & \textbf{100} &30 &39& \textbf{85}&51&24 \\
%     Ours &50 & 88 &\textbf{55} &\textbf{66}& 79& \textbf{69}&13 \\
    
%     \bottomrule
%     \end{tabular}
%      \caption{Cell and header matching results. GO stands for GraphOTTER and TRAG stands for TableRAG. ORI stands for original full table. Apart from precision, recall and $F_1$ , we also show the average number of extracted cells for each system. The gold annotation has an average of 11 cells. \label{tab:sub_table_results}}
% \end{table}


% \subsection{Adding back Relevant Information}
% In this section, we explore different methods of adding back relevant information. \textit{rc}: we prompt the model to focus on relevant columns identified. \textit{rt} we only input the relevant cells in text format to MLLMs. \textit{ri}: we convert the relevant cells into images and pass it to models. \textit{rt+ri}, we feed both relevant cells in texts and images to models. As passing only relevant cells can result in information loss. We consider adding back original tables. \textit{ri+t} encodes relevant cells into image format and original table text into text format and passes both sources of information to MLLMs. \textit{rt+i} encodes relevant cells into text and original table into image and pass both information to models. Results are shown in Figure \ref{fig:add_back_results}.

% We find several observations from Figure \ref{fig:add_back_results}. First, passing relevant cells instead of full table enhance performance. For instance, passing relevant cells predicted from our proposed method results in EMs of 26.55 and 54.11 for (big) reasoning and (big) retrieve settings, respectively. However, the numbers are only 18.69 and 48.10 when passing full table texts to MLLMs.
% Second, again we observe that for reasoning questions, passing both sub-tables as texts and images achieves the best performance. In contrast, for retrieval questions, passing sub-table as text suffices. The pattern applies when using gold and predicted relevant cells to construct sub-tables.
% Thirdly, we find simply pointing out which columns to focus in the prompt to MLLMs does not work as passing relevant cells directly. This might be because higher resolution tables result in long inputs and the encoded linkages between columns might not be informative enough for models to figure out which cells belong to which columns.


% \begin{figure}[htb]
%     \includegraphics[width=1.\linewidth]{images/add_back_results.pdf}
%     \caption{Comparing the effectiveness of different methods of adding back relevant information. Only results for big tabls are shown. Gold refers to using gold relevant cells and Pred refers to using our proposed method to obtain relevant cells. rc stands for encoding relevant columns into the prompt. ri and rt represents passing only relevant image and text, respectively. ri+t stands for passing both relevant cells as image and full table as text. Similarly, rt+i refers to the method of passing relevant cells as text and passing original table as image. Lastly, rt+ti stands for passing both relevant cells as text and image. We employ the Exact Match (EM) metric.}
%     \label{fig:add_back_results}
% \end{figure}

% \paragraph{Take-away messages}
% We propose a method that effectively retrieves relevant cells from tables. Our methods achieves better $F_1$ scores in terms of both cell and header matching than previous SoTA model TableRAG and GraphOTTER. We investigate different ways of injecting relevant table information back to MLLMs, and find passing relevant cells as text when instances featuring retrieval questions and passing relevant cells as both texts and images when the questions are reasoning questions. The observation aligns with what we find previously in Section \ref{sec:results}. 


Table \ref{tab:qa_results} presents the results averaged across three runs. The first section of the table compares direct inference with MLLMs and the application of our framework. The second section of the table compares our method with two SoTA systems using the same model. For the first question, we observe performance improvements after applying our framework, most notably on the HiTab dataset, where an additional 17.5 Exact Match (EM) is achieved when using our method. For the second question, our framework outperforms both SoTA models across all four datasets. Additionally, we observe performance gains after applying our framework on Qwen2 72b on three out of four datasets, although the gains are smaller compared to those on smaller models. We suspect this might be due to the larger models' capabilities of handling longer and more complex instances.




% \begin{table}[htb]
%     \scriptsize
%     \centering    
 
%     \begin{tabular}{*{5}{l}}
%     \toprule
%     Systems & WTQ & TabFact& HiTab & WiKiSQL \\
%     \midrule
%     Pixtral (12b)&51.3 & 75.7 & 59.7 & 58.8 \\
%     +proposed & 54.4 \tiny (\textcolor{teal}{+3.1})&76.8 \tiny (\textcolor{teal}{+1.1}) &68.0 \tiny (\textcolor{teal}{+8.3})&62.7 \tiny (\textcolor{teal}{+3.9}) \\
%     TableLlaVA (7b)&34.4 & 63.7 &44.3  &47.8 \\
%     +proposed &39.7\tiny (\textcolor{teal}{+5.3}) & 64.5 \tiny (\textcolor{teal}{+0.8})&61.8 \tiny (\textcolor{teal}{+17.5})& 52.0 \tiny (\textcolor{teal}{+4.2})\\
%     \midrule
%     Qwen2 (72b) &62.6 & \textbf{86.7}& 73.4& 77.6\\
%     +Proposed & \textbf{63.4}&86.0 &\textbf{76.4} & \textbf{78.0}\\
%     TableRAG & 60.8 & 79.3 & 65.3 & 77.9\\
%     GraphOTTER & 59.4 & 81.8 & 71.6 & 75.6\\
    
    
%     \bottomrule
%     \end{tabular}
%        \caption{Model performances on four TQA benchmarks. The first section (first four rows) shows results of direct inference with MLLMs and applying our framework. The second section (last four rows) compares our framework with two SoTA systems using the same model. \label{tab:qa_results}}
% \end{table}


\begin{table}[htb]
    \small
    \centering    
 
    \begin{tabular}{*{5}{c}}
    \toprule
    System & 0-50 & 50-100& 100-200&>200 \\
    &187& 413 &466&518 \\ 
    \midrule
    MLLM& 64.7&61.2  &60.2&56.4 \\
    + st &+4.1&+5.3&+4.9&+7.5  \\
    + st+qc &+5.9 &+6.9&7.4&+11.1  \\
    
    \bottomrule
    \end{tabular}
       \caption{Ablation study of our framework on HiTab dataset using Pixtral 12b. Results are obtained by averaging the performance of Pixtral 12b on three runs. st stands for sub-table retriever and qc stands for question classifier.\label{tab:system:analysis}}
\end{table}

\paragraph{Ablation} We analyze the contributions of different components within the framework. Additionally, results are segmented based on various table sizes to assess the capabilities of the model and its components across different table sizes. We present results on the HiTab dataset in Table \ref{tab:system:analysis}. HiTab is selected for the ablation study due to its largest performance gains after applying our framework. We find that both components enhance the performance of the overall framework; however, the sub-table retriever has a more substantial impact compared to the question classifier. Regarding table sizes, we observe a decline in system performance as table size increases. Notably, the effectiveness of the sub-table retriever is more pronounced in larger tables compared to smaller ones.



\paragraph{Sub-table Retrieval}
For both LLMs and MLLMs, their performance suffers in cases of long inputs \citep{lin-etal-2023-inner, Wang2024MultimodalNI}. In TQA, to enable models to manage large tables, previous research has proposed various methods for retrieving sub-tables relevant to the questions. These methods fall into two categories: fine-tuned retrievers \cite{lin-etal-2023-inner,Lee2024PieceOT} and LLM-based retrievers \cite{Chen2024TableRAGMT, Li2024GraphOTTEREL,10.1145/3539618.3591708}. The former involves training a smaller model using gold sub-table annotations, while the latter capitalizes on the capabilities of LLMs through few-shot demonstrations. Although LLM-based approaches avoid the challenges of acquiring additional gold sub-table data, their performance may be hindered when faced with complex questions or large tables. In this study, we propose a straightforward yet effective method for retrieving sub-tables. This approach integrates a question parser to decompose complex questions and includes a coder to ensure accurate sub-table retrieval.

\paragraph{MLLMs for TQA} In TQA, most previous research treat tables as text \citep{Zhang2023TableLlamaTO,Wang2024ChainofTableET}, employing LLMs to tackle the task. \citet{zheng-etal-2024-multimodal} introduce the concept of multi-modal table understanding, where tables are processed as images. Given that tables can exist in both formats in real-world scenarios and that these two formats are interconvertible (table text to image via HTML rendering, table image to text using Optical Character Recognition tools), it naturally raises the question of how to harness both formats to achieve performance gains. To our knowledge, no prior work has investigated this question. In this work, we propose a framework that utilizes both formats to enhance task performances.


% \paragraph{Table Structure}
% Table images retain structural information better than table texts, where structure is lost during parsing.
% As a result, one might assume MLLM with table image is more suitable for tables with complex structures than LLM with table texts.
% To test this hypothesis, we can evaluate MLLM and LLM on hierarchical tables. 

%Running additional evaluations on the flattened hierarchical tables might reveal challenges in coping with complex table structure. 
%However, the flattening process enlarges table size by duplicating hierarchical headers, causing differences in both structure and size.
%We therefore only look at the hierarchical setting when comparing MLLMs and LLMs. 

% \paragraph{Input}
% Table related tasks sometimes can involve more than just one single table. For instance, Spider (cite) features querying over multiple tables and FinQA (cite) requires joint reasoning over table and texts.
% We therefore examine MLLMs and LLMs on these settings to see if there exists any preference of the models.

% \paragraph{Tasks}
% The two most common setups for table related tasks are question answering and data-to-text summarization. 
% We therefore explore how do the performance of MLLMs and LLMs differ on these different tasks.
% For data-to-text summarization, we focus on highlighted cells summarization, as the color encoding of cells in table image might provide additional advantage to MLLM. 

% \begin{figure*}
%     \includegraphics[width=1.\linewidth]{images/system_overview.pdf}
%     \caption{System overview. Given a table and question pair, a sub-table retriever outputs a shorted version of the table. A question classifier is applied to distinguish retrieval and reasoning question. Based on the question type, a table reformatter prepares input table for the table reasoner, which outputs final answer based on shorted table and a question. \anne{sorry for asking again: is the robot the LLM?}}
%     \label{fig:system}
% \end{figure*}
% We now investigate: \textit{How can we leverage our findings for further performance gains?} \heiketodo{this sentence plus question does not really fit to the style of the rest of the paper} 

==> latex/related_work.tex <==
% \section{Related Work}
% \heiketodo{remove paragraph heading (if there is only one paragraph)}
% \paragraph{Table as Text and Table as Image}
%  \citet{deng-etal-2024-investigating} compares MLLMs using table image representation and LLMs using table text representation on various TQA datsets, finding similar performance. %They find MLLMs using image representations competitive to LLMs with table text representation.
%  However, they did not look into the impact of data on performance. For instance, MLLMs might not process large (high resolution) table \heiketodo{table images with many pixels?} as well as LLMs, due to its bottleneck of dealing with high resolution images \citep{Li2023MonkeyIR}. 
%  Additionally, since MLLMs is able to take both image and text (given both exist), it is unclear if representation matters to performance. 
%  To this end, we compare between models and between table representations in four settings where question complexity and table sizes vary. \annetodo{this paragraph seems to fit better as the gap in the intro}
%  \heiketodo{agree; apart from that, a related work section with only two works is not enough}
 
% \label{sec:rel}
%

==> latex/results.tex <==
%\section{Results}
%\label{sec:results}
%
